An Empirical Study on Finding Spans

We present an empirical study on methods for span finding, the selection of consecutive tokens in text for some downstream tasks. We focus on approaches that can be employed in training end-to-end information extraction systems, and find there is no definitive solution without considering task properties, and provide our observations to help with future design choices: 1) a tagging approach often yields higher precision while span enumeration and boundary prediction provide higher recall; 2) span type information can benefit a boundary prediction approach; 3) additional contextualization does not help span finding in most cases.

==> sections/appendices/dataset_stats.tex <==

\subsection{ACE Statistics}
\begin{table}[h]
\resizebox{\linewidth}{!}{%
    \centering
    \begin{tabular}{lcccccc}
      \toprule
         & \multicolumn{3}{c}{ACE05-R} & \multicolumn{3}{c}{ACE05-E\textsuperscript{+}} \\
         \cmidrule(lr){2-4}\cmidrule(lr){5-7}
         & Train & Dev & Test & Train & Dev & Test \\
      \midrule
      \#Instances & 8486 & 2031 & 1733 & 19181 & 901 & 676 \\
      \#Entities & 26470 & 6402 & 5476 & 47452 & 3423 & 3673 \\
      \#Relations & 4781 & 1177 & 1149 & 7154 & 728 & 802 \\
      \#Events & - & - & - & 4419 & 468 & 424 \\
      \bottomrule
    \end{tabular}
    }
    \caption{Summary statistics for ACE05 dataset}
    \label{tab:ace_stats}
\end{table}

\subsection{SQuAD 2.0 Statistics}
\begin{table}[h]
    \centering
    \resizebox{0.6\linewidth}{!}{%
    \begin{tabular}{l|cc}
      \toprule
         & Train &Dev \\
      \midrule
         \#Answerable & 86821 & 5928 \\
         \#Unanswerable & 43498 & 5945 \\
      \bottomrule
    \end{tabular}
    }
    \caption{Summary stats for the SQuAD2.0 dataset.}
    \label{tab:SQuAD_stats}
\end{table}

==> sections/appendices/detailed_setup.tex <==
\paragraph{EE, RE, and NER}

%Reason to use OneIE over DYGIE, I am not sure whether this is the correct place that I should place this
%We chose OneIE as our baseline for NER, RE, and EE because that it is well-known to the IE community and it is a strong baseline for these tasks with open source access. In addition, compared to other SoTA models that jointly train the span finding module via the downstream modules like DYGIE, OneIE trains the span finding module only with the objective of span extraction, which provides the flexibility to better serve our purpose of only replacing the span finding module without introducing modifications to other components.

\paragraph{Coreference Resolution}


\paragraph{Question Answering}

==> sections/appendices/full_experiments.tex <==

% \paragraph{SQuAD 2.0 Results}
% \begin{table}[h]
% \resizebox{\linewidth}{!}{%
%     \centering
%     \begin{tabular}{l|cc}
%       \toprule
%         \bf Approach & \bf EM & \bf F\textsubscript{1}\\
%       \midrule
%         CRF(RoBERTa\textsubscript{base}) & 74.4  & 80.8\\
%         +BiLSTM & 74.7 & 81.3\\
%         CRF(T5\textsubscript{base}) & 58.1  & 67.3\\
%         +BiLSTM & 62.1 & 70.7\\
%       \midrule
%         Boundary Prediction(RoBERTa\textsubscript{base}) &77.6 & 85.0\\
%         +BiLSTM & 78.1 & 85.4\\
%         Boundary Prediction(T5\textsubscript{base}) &70.3 &76.1\\
%         +BiLSTM & 73.9 & 79.9\\
%       \midrule
%         Span Enumeration(RoBERTa\textsubscript{base}) &68.8 &73.8\\
%         +BiLSTM & 68.7 & 73.9\\
%         Span Enumeration(T5\textsubscript{base}) & 62.3 & 66.1\\
%         +BiLSTM & 63.6 & 67.1\\
%       \bottomrule
%     \end{tabular}
%     }
%     \caption{Full experiment results on SQuAD 2.0 dev set.}
%     \label{tab:qa_exps}
% \end{table}

%\begin{table*}[h]
% \resizebox{\textwidth}{!}{%
%     \centering
%     \begin{tabular}{l|cccccccccccccccc}
%       \toprule
%         \bf Approach & \multicolumn{3}{c}{\bf Macro} & \multicolumn{3}{c}{\bf MUC} & \multicolumn{3}{c}{\bf B\textsuperscript{3}}& \multicolumn{3}{c}{\bf CEAF} & \multicolumn{3}{c}{\bf Mention} \\
%         \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
%          & Prec & Rec & \bf F\textsubscript{1}& Prec & Rec & \bf F\textsubscript{1}& Prec & Rec & \bf F\textsubscript{1} & Prec & Rec & \bf F\textsubscript{1}& Prec & Rec & \bf F\textsubscript{1}& \\
%       \midrule
%         CRF(RoBERTa\textsubscript{base}) &63.2&	48.1&	54.0&	72.8&	63.2&	67.7&	56.3&	49.3&	52.6&	60.4&	31.8&	41.6&	80.1&	73.7&	76.8 \\
%         +BiLSTM &63.6&	48.4&	54.2&	73.2&	63.5&	68.0	&56.3&	50.0&	53.0&	61.4&	31.6&	41.7	&81.2	&73.3	&77.0  \\
%         -Overlap &63.0&	49.4&	54.5&	72.5&	64.6&	68.3&	54.5&	51.4&	52.9&	61.9	&32.1&	42.3&	81.7	&72.8&	77.0  \\
%         -Overlap+BiLSTM &61.8&	52.0&	55.4	&70.5&	67.4&	68.9&	52.7&	55.4&	54.0	&62.3&	33.3	&43.4&	79.3	&75.6	&77.4   \\

%         CRF(T5\textsubscript{base}) &66.6	&59.2&	62.3&	72.8&	70.0	&71.4&	59.9&	60.1&	60.0&	67.1&	47.4&	55.6&	78.5&	76.3&	77.4  \\
%         +BiLSTM &60.4	&51.9&	54.7&	69.4&	67.2&	68.3	&50.9&	55.7	&53.2	&60.7&	32.7&	42.5&	78.8&	75.7&	77.2\\
%         -Overlap &61.3&	52.1&	55.1&	70.4&	67.7&	69.0&	51.5&	56.2&	53.7&	62.0&	32.3&	42.5&	79.4	&76.0&	77.7\\
%         -Overlap+BiLSTM &66.1&	48.0&	55.2&	75.6&	62.3	&68.3&	61.5&	47.5&	53.6&	61.2&	34.0&	43.8&	80.9&	73.2&	76.8\\

%       \midrule
%         Boundary(RoBERTa\textsubscript{base}) &74.8&	71.5&	73.1&	82.1&	78.7&	80.4&	72.8&	69.6&	71.1&	69.3	&66.3&	67.8&	28.1&	95.4&	43.4\\
%         +BiLSTM &73.6&	70.8&	72.1&	81.2&	80.5&	80.8&	71.1&	72.1&	71.6&	68.6&	59.8&	63.9&	25.4&	95.5&	40.1\\
         % +BiLSTM &74.75&	71.5&	73.09	&82.14&	78.69&	80.38&	72.79&	69.55&	71.14&	69.31&	66.26&	67.75&	28.07&	95.38&	43.38\\
%         -Overlap &72.4	&71.2&	71.7&	80.1&	80.7&	80.4&	69.3&	72.6&	70.9&	67.8	&60.1	&63.7&	25.5&	96.0&	40.3\\
%         -Overlap+BiLSTM &74.1&	70.9&	72.3&	81.3&	80.8	&81.1&	71.4&	72.2&	71.8&	69.5&	59.6&	64.2&	25.5&	95.7	&40.2\\

%         Boundary(T5\textsubscript{base}) &67.6&	67.6&	67.5&	74.7&	76.3&	75.5&	62.7&	67.4&	65.0&	65.5&	59.1&	62.1&	25.0&	96.3&	39.7\\
%         +BiLSTM & 74.3&	69.7&	71.8&	82.1&	80.2&	81.1&	71.0&	70.3&	70.6&	69.7&	58.6&	63.7&	25.8&	97.0&	40.7\\
%         -Overlap&71.6	&69.7	&70.5&	79.5&	79.8&	79.6&	67.4&	70.5&	68.9&	67.8	&58.7&	62.9&	25.8&	96.9&	40.7\\
%         -Overlap+BiLSTM &72.9	&70.6	&71.6&	80.5&	80.9&	80.7&	68.9&	71.6&	70.2&	69.3&	59.2&	63.8&	25.8&	97.0&	40.8\\

%       \midrule
%         Enumeration(RoBERTa\textsubscript{base})  &71.2&	67.2&	69.1&	77.6&	75.6&	76.6&	68.6&	66.0&	67.3&	67.4&	59.9&	63.5&	25.0&	96.4&	39.7\\
        
%         +BiLSTM &71.8&	67.1	&69.3	&78.1	&75.7	&76.9	&68.9&	66.0&	67.4&	68.3&	59.6&	63.6&	24.9&	95.9&	39.5\\
        
%         -Overlap &73.91&	71.2	&72.5&	81.0&	81.0&	81.0&	71.4&	72.4&	71.9&	69.3&	60.3&	64.5&	25.5	&96.1	&40.4\\
        
%         -Overlap+BiLSTM& 74.5&	70.6&	72.4&	81.8&	80.6&	81.2&	72.0	&72.1&	72.0&	69.8&	59.1&	64.0&	25.5&	96.0&	40.3\\

%         Enumeration(T5\textsubscript{base})& 67.2&	67.2&	67.1&	74.3&	76.2&	75.2&	61.9&	66.9&	64.3&	65.3&	58.5&	61.7&	25.0&	96.3&	39.7\\
%         +BiLSTM &71.1	&66.9	&68.9	&78.1&	75.4&	76.7	&68.1&	65.5&	66.7&	67.1&	59.8&	63.3	&25.1&	96.5&	39.8\\
%         -Overlap &72.3	&68.7	&70.4&	80.3&	79.1&	79.7&	68.7&	69.0&	68.8&	67.9&	58.1	&62.6&	25.6&	96.4&	40.5\\
%         -Overlap+BiLSTM &71.5&	71.0&	71.3&	79.5&	78.4&	78.9&	67.7&	69.7&	68.7&	67.4	&64.9	&66.1&	28.2&	95.8&	43.6\\
%       \bottomrule
%     \end{tabular}
%     }
%     \caption{Full experiment results of coreference resolution task on CoNLL-12 dataset}
%     \label{tab:coref_baseline_exps}
%\end{table*}


% \subsection{Hyperparameter}
% \paragraph{OneIE}


% \paragraph{Coreference Resolution}

% \paragraph{Question Answering}

==> sections/appendices/mention_breakdowns.tex <==
 % This is the breakdown for the mention scores of OneIE, I am not sure where to add the table as well
 % I included entity mention and event mention(triggers)
 % Reminder: We used the model that without the additional typing layer as our baseline
\begin{table*}[h]
\resizebox{\linewidth}{!}{%
    \centering
    \begin{tabular}{l|cccccccccccc}
       \toprule
        \bf Approach & \multicolumn{3}{c}{\bf Entity-I} & \multicolumn{3}{c}{\bf Entity-C} & \multicolumn{3}{c}{\bf Trigger-I}& \multicolumn{3}{c}{\bf Trigger-C}\\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
         & Prec & Rec & \bf F\textsubscript{1}& Prec & Rec & \bf F\textsubscript{1}& Prec & Rec & \bf F\textsubscript{1} & Prec & Rec & \bf F\textsubscript{1}\\
        \midrule
        Tagging (RoBERTa\textsubscript{base}) & 94.5 & 94.8 & 94.6 & 89.9 & 90.1 & 90.0 & 70.9 & 76.0 & 73.3 & 65.5 & 72.7 & 68.9\\
        Tagging (T5\textsubscript{base}) & 93.9 & 95.0 & 94.5 & 90.7 & 89.0 & 88.6 & 71 & 52.6 & 60.2 & 46.6 & 33.7 & 39.0\\
        \midrule
        Boundary Prediction (RoBERTa\textsubscript{base}) & 94.9 & 94.9 & 94.9 & 90.1 & 89.6 & 89.9 & 71.4 & 73.3 & 72.3 & 67.2 & 68.2 & 67.7 \\
        Boundary Prediction (T5\textsubscript{base}) & 95.6 & 95.4 & 95.5 & 90.7 & 90.3 & 90.5 & 69.4 & 72.0 & 70.7 & 67.5 & 69.3 & 68.3\\
        \midrule
        Span Enumeration (RoBERTa\textsubscript{base}) & 94.1 & 95.4 & 94.8 & 89.3 & 90.2 & 89.7 & 65.9 & 81.0 & 72.7 &62.5 &77.1 & 69.0\\
        Span Enumeration (T5\textsubscript{base}) & 88.6 & 95.6 & 92.0 & 83.1 & 89.6 & 86.2 & 45.1 & 86.2 & 59.2 & 36.4 & 69.5 & 47.8 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Breakdowns for the mention scores.}
    \label{tab:mention_breakdown}
\end{table*}
